Learnable Topological Features for Phylogenetic Inference via Graph Neural Networks

Structural information of phylogenetic tree topologies plays an important role in phylogenetic inference. However, finding appropriate topological structures for specific phylogenetic inference tasks often requires significant design effort and domain expertise. In this paper, we propose a novel structural representation method for phylogenetic inference based on learnable topological features. By combining the raw node features that minimize the Dirichlet energy with modern graph representation learning techniques, our learnable topological features can provide efficient structural information of phylogenetic trees that automatically adapts to different downstream tasks without requiring domain expertise. We demonstrate the effectiveness and efficiency of our method on a simulated data tree probability estimation task and a benchmark of challenging real data variational Bayesian phylogenetic inference problems.

==> rooted_tree.tex <==

% Clade node
\tikzstyle{clade} = [latent, rectangle, minimum size=18pt, node distance=2]

% Leaf node
\tikzstyle{leaf} = [font=\fontsize{15}{15}\selectfont, node distance=2]

% \squaredge  [options]  {inputs}  {outputs}
\newcommand{\squaredge}[3][] {
  % Connect all nodes #2 to all node #3.
  \foreach \x in {#2} {
    \foreach \y in {#3} {
      \draw[semithick, #1]  (\x) -- (\x |- \y) -- (\y);
    };
  };
}

% \csquaredge [options] {inputs} {outputs}
\newcommand{\csquaredge}[3][] {
  % Connect all nodes #2 to all node #3.
  \foreach \x in {#2} {
    \foreach \y in {#3} {
      \draw[semithick, #1]  (\x.center) -- (\x |- \y) -- (\y.center);
    };
  };
}

\newcommand{\undiredge}[5][] {
  % Connect all nodes #2 to all nodes #3.
  \foreach \x in {#4} {
    \foreach \y in {#5} {
      \path (\x.center) edge[#1] node[pos=0.5, below, #2]{#3} (\y.center);
      };
    };
}

\newcommand{\undiredgeleaf}[5][] {
  % Connect all nodes #2 to all nodes #3.
  \foreach \x in {#4} {
    \foreach \y in {#5} {
      \path (\x.center) edge[#1]node[pos=0.5, below, #2]{#3} (\y);
      };
    };
}


% \csquaredgeleaf [options] {inputs} {outputs}
\newcommand{\csquaredgeleaf}[3][] {
  % Connect all nodes #2 to all node #3.
  \foreach \x in {#2} {
    \foreach \y in {#3} {
      \draw[semithick, #1]  (\x.center) -- (\x |- \y) -- (\y);
    };
  };
}

% \annotatededge [options] [options] {edge value} {inputs} {outputs}
\newcommand{\annotatededge}[5][] {
 % Connect all nodes #2 to all node #3
 \foreach \x in {#4} {
   \foreach \y in {#5} {
     \path (\x) edge [->, >={triangle 45}, #1] node [pos=0.5, below, #2] {#3} (\y);
     };
   };
}
   
% \undirannotatededge [options][options] {edge value} {inputs} {outputs}
\newcommand{\undirannotatededge}[5][] {
 % Connect all nodes #2 to all nodes #3
 \foreach \x in {#4} {
   \foreach \y in {#5} {
     \path (\x) edge[#1] node [pos=0.5, below, #2] {#3} (\y);
   };
 };
 }
      


